Decoupling feature extraction from policy learning: assessing benefits of state representation learning in goal based robotics

Scaling end-to-end reinforcement learning to control real robots from vision presents a series of challenges, in particular in terms of sample efficiency. Against end-to-end learning, state representation learning can help learn a compact, efficient and relevant representation of states that speeds up policy learning, reducing the number of samples needed, and that is easier to interpret. We evaluate several state representation learning methods on goal based robotics tasks and propose a new unsupervised model that stacks representations and combines strengths of several of these approaches. This method encodes all the relevant features, performs on par or better than end-to-end learning with better sample efficiency, and is robust to hyper-parameters change.

==> for_future_paper.tex <==
% material for future paper, extension of this one
 %% ON DUAL CAMERA:
Fig. \ref{fig:learning-curve-dual-cam} shows that the use of multiple camera views demonstrated to provide higher RL performance on static targets (\textit{Kuka-arm-button}) such that, without (moving) distractors, performance of (V)AE dual view is higher than single views. With respect to objective functions, in the same setting, the triple loss-based model as in Time Contrastive Networks (TCN) \citep{Sermanet17} gives better average rewards than robotic priors loss functions.

However, overall, with and without distractors, plots in Fig. \ref{fig:learning-curve-dual-cam} show that convergence speed is slightly boosted with dual cameras. When applying robotic priors, however, the gain in performance by using dual camera images stacked does not show significant improvement w.r.t. a single view.

\begin{figure}[htbp!]
 \centering 
 \includegraphics[scale=0.2]{images/learning-curve-dual-cam}
 \caption{Left: The impact of adding a second view through a triplet loss as in TCN \citep{Sermanet17}. Right: Performance of Forward, Inverse and Forward+Inverse models \cnat{TODO: add plot: best models including reward prediction too if possible?)}}
 \label{fig:learning-curve-dual-cam}
\end{figure}


We also showed that useful modules in state representation learning include, among others, the addition of a second view dual camera using a triplet loss (either with (V)AE \citep{Baldi12}, ResNet18 \citep{He15}). 


\begin{table} [htbp!]
\caption{Datasets and environments for state representation learning. %Input image size and output state dimensionality are described, as well as the cardinal and nature of the actions
}
\label{tab:environments} 
\begin{tabular}[htbp!]
{llll} \hline Environment & Task objective & Nr. Actions & Input image\\ \hline %image size  \\\hline
      
1- \textit{Mobile-robot-band} & Reach (\textit{park}) on band area & 4, Discrete & 224x224 \\ % \\% & Abs. \& rel. pos. of robot, dist. to target. \\
2- \textit{Mobile-robot-navigation} & Reach (\textit{park}) on button area & 4, Discrete & 224x224\\ %Fixed and mobile & Abs. \& rel. pos. of robot  \\
3- \textit{Kuka-arm-button} & Push button & 5, Discrete & 224x224 \\ % & Abs. \& rel. pos. of hand gripper\\ 
4- \textit{Baxter-arm-button} & Push button & 5, Discrete & 224x224 \\ %Fixed and mobile & Abs. \& rel. pos. of hand gripper \\  
      \hline
  \end{tabular}
\end{table}





\begin{table} [htbp!]
\begin{tabular}{ lllllll}\hline 
\centering Static/Random Target & \multicolumn{3}{c}{Absolute position } & \multicolumn{3}{c}{Relative position} \\
\centering Mobile robot (1) & \multicolumn{2}{c}{KNN-MSE}  & Avg. reward & \multicolumn{2}{c}{KNN-MSE}  & Avg. reward 
\\\hline  
\centering \textit{GT}  & 0.0099  & \multicolumn{2}{c}{ $\pm$ }  & 0.0164  & \multicolumn{2}{c}{$\pm$  }  \\ 
\centering \textit{Supervised} & 0.0164 & \multicolumn{2}{c}{ $\pm$ } & 0.0306   & \multicolumn{2}{c}{ $\pm$ } \\
\centering \textit{AE} & 0.0168  & \multicolumn{2}{c}{ $\pm$ } & 0.7213  & \multicolumn{2}{c}{ $\pm$ }      \\ 
\centering \textit{VAE} & 0.0161  & \multicolumn{2}{c}{ $\pm$ } &   0.1295  & \multicolumn{2}{c}{ $\pm$ }    \\
\centering \textit{Robotic Priors} & 0.0200 & \multicolumn{2}{c}{ $\pm$ } & 0.0900  & \multicolumn{2}{c}{ $\pm$ }  \\
\centering \textit{Forward} & 0.5111  & \multicolumn{2}{c}{ $\pm$ }  & 1.1557  & \multicolumn{2}{c}{ $\pm$ }      \\
\centering \textit{Inverse} & 0.0191  & \multicolumn{2}{c}{ $\pm$ } & 0.7703  & \multicolumn{2}{c}{ $\pm$ }  \\
 \centering \textit{Fwd+Inv} &  0.0164 & \multicolumn{2}{c}{ $\pm$ } & 0.7467  & \multicolumn{2}{c}{ $\pm$ }  \\
% \centering \textit{Fwd+Inv+Rew.Prediction} & 0.0168  & 0.6427  & 0.0275  &  0.1241  & 0.0376 \\%& NA  \\ FUTURE: TODO
\hline 
\end{tabular}
\caption{KNN-MSE and mean reward performance in RL per episode with standard error for each SRL method. GT (robot absolute or relative position with respect to target object), forward (fwd), inverse (inv) models and combinations in mobile robot navigation environment.}
\label{tab:knn-mse-rewards-per-episode}
\end{table}



Conclusions
Furthermore, an extra experimental setting includes the addition of images from a second point of view camera from the same timestep but different view as positive samples, while different timesteps are set apart from a given input anchor image \citep{Sermanet17}. 




%older versions of tables
\begin{table} [htbp!]
 \centering 
\begin{tabular}{ llll}\hline 
\centering Mobile robot (1) & \multicolumn{2}{c}{KNN-MSE}  & Avg. reward 
\\\hline  
\centering \textit{GT}  & 0.0099  & \multicolumn{2}{c}{ $\pm$ } \\ 
\centering \textit{Supervised} & 0.0164 & \multicolumn{2}{c}{ $\pm$ }  \\
\centering \textit{AE} & 0.0168  & \multicolumn{2}{c}{ $\pm$ } \\ 
\centering \textit{VAE} & 0.0161  & \multicolumn{2}{c}{ $\pm$ }  \\
\centering \textit{Robotic Priors} & 0.0200 & \multicolumn{2}{c}{ $\pm$ } \\
\centering \textit{Forward} & 0.5111  & \multicolumn{2}{c}{ $\pm$ } \\
\centering \textit{Inverse} & 0.0191  & \multicolumn{2}{c}{ $\pm$ } \\
 \centering \textit{Fwd+Inv} &  0.0164 & \multicolumn{2}{c}{ $\pm$ } \\
\hline 
\end{tabular}
\caption{KNN-MSE and mean reward performance in RL per episode with standard error for each SRL method. GT (robot absolute position with respect to target object), forward (fwd), inverse (inv) models and combinations in mobile robot (absolute target position) navigation environment.}
\label{tab:knn-mse-rewards-per-episode}
\end{table}




% In terms of convergence speed up in RL training, even if they are only useful during simulation and do not work with goals that move in between episodes, CMA-ES and ARS are the (ES) algorithms to use in the RL phase. 


% \subsubsection{Reward diversity and predicting reward}

% Reward diversity is important and, generally, imposed by the formulation of the task, e.g., see robotic priors \citep{Jonschkowski15}. We noticed that providing more reward diversity, i.e., having a negative reward value apart from null and positive ones, seems to help, specially in our cases where reward is normally sparse (only seen after many steps, at the end of the episode). In such example, for instance, having the robot to bump into walls results in a reward value of -1 \citep{Jonschkowski15}, which also helps for real robots safety. 

% When using combination of approaches, the inverse-forward module architecture can optionally include a reward prediction model's categorical (cross entropy) loss term \cnat{precise if other function tested worked best?} $\mathcal{L}_{rw} = r_{t+1} - \hat{r}_{t+1}$. 

%By using our proposed tools we can observe that SRL is able to successfully learn absolute positions of controlled objects (e.g., states that represent the mobile robot position or the robot arm position). However, the models exhibit difficulties at learning relative positions of the robot/end effector with respect to the target object to be reached. 
%Simple robot control task experiments show that it is better to apply forward and inverse models together than each of them separately. Optionally, adding a module where reward is predicted, seems to hurt the interpretability or intuitive geometry of the state space learned.


